DNNFusion: Accelerating Deep Neural Networks Execution with Advanced Operator Fusion

Deep Neural Networks (DNNs) have emerged as the core enabler of many major applications on mobile devices. To achieve high accuracy, DNN models have become increasingly deep with hundreds or even thousands of operator layers, leading to high memory and computational requirements for inference. Operator fusion (or kernel/layer fusion) is key optimization in many state-of-the-art DNN execution frameworks, such as TensorFlow, TVM, and MNN. However, these frameworks usually adopt fusion approaches based on certain patterns that are too restrictive to cover the diversity of operators and layer connections. Polyhedral-based loop fusion techniques, on the other hand, work on a low-level view of the computation without operator-level information, and can also miss potential fusion opportunities. To address this challenge, this paper proposes a novel and extensive loop fusion framework called DNNFusion. The basic idea of this work is to work at an operator view of DNNs, but expand fusion opportunities by developing a classification of both individual operators and their combinations. In addition, DNNFusion includes 1) a novel mathematical-property-based graph rewriting framework to reduce evaluation costs and facilitate subsequent operator fusion, 2) an integrated fusion plan generation that leverages the high-level analysis and accurate light-weight profiling, and 3) additional optimizations during fusion code generation. DNNFusion is extensively evaluated on 15 DNN models with varied types of tasks, model sizes, and layer counts. The evaluation results demonstrate that DNNFusion finds up to 8.8x higher fusion opportunities, outperforms four state-of-the-art DNN execution frameworks with 9.3x speedup. The memory requirement reduction and speedups can enable the execution of many of the target models on mobile devices and even make them part of a real-time application.

==> tex/cases.tex <==
\section{Case Study}
\textcolor{cyan}{Showing the case study of common fusion combination}

\subsection{CONV case study}

\subsection{GEMM case study}

\subsection{Broadcast case study}

\subsection{Concat case study}

\begin{figure}[t]
    \centering
        \subfloat[CONV on CPU.]{
            \includegraphics[width=0.48\columnwidth]{evaluation/Case_CONV_CPU.pdf}
        }
        \subfloat[CONV on GPU.]{
            \includegraphics[width=0.48\columnwidth]{evaluation/Case_CONV_GPU.pdf}
        }
        \caption{{\bf Case study - CONV on mobile devices.}}
    \label{fig:case_conv}
\end{figure}

\begin{figure}[t]
    \centering
        \subfloat[GEMM on CPU.]{
            \includegraphics[width=0.48\columnwidth]{evaluation/Case_Gemm_CPU.pdf}
        }
        \subfloat[GEMM on GPU.]{
            \includegraphics[width=0.48\columnwidth]{evaluation/Case_Gemm_GPU.pdf}
        }
        \caption{{\bf Case study - GEMM on mobile devices.}}
    \label{fig:case_gemm}
\end{figure}

\begin{figure}[t]
    \centering
        \subfloat[Broadcast on CPU.]{
            \includegraphics[width=0.48\columnwidth]{evaluation/Case_Broadcast_CPU.pdf}
        }
        \subfloat[Broadcast on GPU.]{
            \includegraphics[width=0.48\columnwidth]{evaluation/Case_Broadcast_GPU.pdf}
        }
        \caption{{\bf Case study - Broadcast on mobile devices.}}
    \label{fig:case_broadcast}
\end{figure}

\begin{figure}[t]
    \centering
        \subfloat[Concat on CPU.]{
            \includegraphics[width=0.48\columnwidth]{evaluation/Case_Concat_CPU.pdf}
        }
        \subfloat[Concat on GPU.]{
            \includegraphics[width=0.48\columnwidth]{evaluation/Case_Concat_GPU.pdf}
        }
        \caption{{\bf Case study - Concat on mobile devices.}}
    \label{fig:case_concat}
\end{figure}

==> tex/design-old-bak.tex <==
\section{\projectname Code Optimization}



\subsection{Light Profile-driven Fusion Plan Exploration}



\subsubsection{Overall Idea of Fusion Plan Exploration}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98 \columnwidth]{figures/fusion_plan_generation.pdf}
    \caption{{\bf An example of fusion plan exploration.} For simplicity, we suppose {\tt Add, Conv, Relu, Mul, Sub} have the same output shape, that means they also have the same IRS size.}
    \label{fig:fusion-plan-generation}
\end{figure}



% https://www.overleaf.com/learn/latex/code_listing
\lstset{numbers=left, numberstyle=\tiny, stepnumber=1, numbersep=5pt, frame=tb, caption=Fusion plan generation,emph={IR_deletable},emphstyle=\underbar}
\lstinputlisting[label={lst:fusion-plan-generation},language=python]{codes/plan-generation.py}

Optimal fusion plan generation usually requires a large (exponential) search space~\cite{elgamal2017spoof, boehm2018optimizing}
and has been shown to be  NP-complete~\cite{kennedy1993maximizing, darte1999complexity}.
To keep the process at manageable costs,  \projectname  explores fusion plans by employing 
a new light-weight (greedy) approach based on our proposed Extended Computational Graph IR and the abstracted mapping types. 


\begin{table}
\caption{{\bf Mapping type analysis.} The first row and column without color show the mapping types of two operators before fusion, and the colored cells show the mapping type of the operator after fusion. Green implies that   these fusion combinations can be fused directly (i.e., legal and likely profitable). 
Red  implies that these fusions are illegal \gagrawal{check if that is correct?}  Yellow implies legal but that  further profiling is required to determine profitability. }
\label{tab:mapping-type-lookup}
\centering
\includegraphics[width=0.98\columnwidth]{figures/mapping_type_combo.pdf}
\end{table}

\gagrawal{choose an abbreviation for Extended Computational Graph and use that everywhere}
 
The key features of our heuristic exploration  include:
First, \projectname selects the starting operators (called {\em fusion seed operators}) from our Extended Computational Graph  to restrict search space. This is based on a key insight  
which is that operations of  one-to-one mapping type have the  potentially to yield more benefits because they a) consume the least number of registers and have lower memory  
requirements among all mapping types, and b) potentially result in fusion of more layers, including   both with  their predecessors and successors because of their most straightforward mapping between input and output tensors \textcolor{blue}{TODO: check this}. 
%
Second, starting with these seed operators, \projectname explores fusion opportunities along with two directions  recursively, i.e., the seed operators' successors (producers) 
direction and producers (predecessors)  direction.
%
Third, \projectname creates fusion plans based on an integrated cost analysis that combines machine-independent mapping type analysis and a 
profiling method with a {\em historical profiling result database}. The mapping type analysis follows Table~\ref{tab:mapping-type-lookup} to check the operators' mapping type combination (in the Extended Computational Graph) to decide if these operators should be fused. \textcolor{red}{TODO: How to justify this table? How to get it?} \gagrawal{The table definitely needs more 
explanation} 
\bren{TODO: a benefit explanation of this combined method: Mapping type analysis eliminates unnecessary profiling thus saving time. Profiling-based approach is more accurate than analytic cost models because of the complicated interplay between DNN execution and hardware configurations~\cite{} ANY CITE. The historical database consisting of profiling results with common fusion patterns further accelerates fusion cost analysis.}


% \textcolor{blue}{Describe why some of them should be fused together while some not.}
% \begin{itemize}
%     \item Register spilling
%     \item Data locality \& cache performance
%     \item Data reuse/compute times
% \end{itemize}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95 \textwidth]{figures/fusion_type_example.pdf}
    \caption{{\bf Examples of graph rewriting with computation properties.} Associative property
    explores the optimal execution order of operators and replaces the expensive combination of operators with a cheaper one.
    Distributive property
    explores the common combination of operators and simplifies the computation structure.
    Commutative property switches the execution order of operators to reduce the overall computation.}
    \label{fig:fusion-type-example}
\end{figure*}

\begingroup
\setlength{\tabcolsep}{5pt}
\begin{table*}[t]
\centering
\caption{{\bf Graph rewriting patterns with computation properties on sub-graphs in each candidate fusion block.} We omit other unrelated operator for better readability. $\odot, +, -, Abs, Recip, Square, \sqrt{\phantom{x}}$ mean element-wise multiplication, addition, subtraction, absolute, reciprocal, square, and square root, respectively. {\tt BitShift} calculates the bit shifted value of elements of a given tensor element-wisely. {\tt ReduceSum} and {\tt ReduceProd} calculate the reduced summation and production of elements of an input tensor along an axis. {\tt Exp} calculates the exponent of elements in a given input tensor element-wisely.}
\label{tab:graph_rewrite_example}
\small
\begin{tabular}{l|cr|cr}
     \toprule
     \multirow{2}{*}{Property} & \multicolumn{2}{c|}{Without graph rewrite} & \multicolumn{2}{c}{With graph rewrite} \\ \cline{2-5}
     ~ &  Graph structure in equation & \#FLOPS & Graph structure in equation & \#FLOPS \\
     \hline
     \multirow{4}{*}{Associative} & $Recip(A) \odot Recip(A \odot B)$ & $4 * m * n$ & $Square(Recip(A)) \odot B$ & $3 * m * n$\\
     ~ & $(A \odot \sqrt{B}) \odot (\sqrt{B} \odot C)$ & $5 * m * n$ & $A \odot B \odot C$ & $3 * m * n$\\
     ~ & $Abs(A) \odot B \odot Abs(C)$ $^\dag$ & $4 * m * n$ & $Abs(A \odot C) \odot B$ & $3 * m * n$\\
     ~ & $(A \odot ReduceSum(B)) \odot (ReduceSum(B) \odot C)$ & $5 * m * n$ & $A \odot Square(ReduceSum(B)) \odot C$ & $3 * m * n$\\
     \hline
     \multirow{3}{*}{Distributive} & $A \odot C$ + $A \odot B$ & $3 * m * n$ & $(A + B) \odot C$ & $2 * m * n$\\
     ~ & $A + A \odot B$ & $2 * m * n$ & $A \odot (B + 1)$ & $m * n$ $\S$ \\
     ~ & $Square(A + B) - (A + B) \odot C$ & $4 * m * n$ & $(A + B) \odot (A + B - C)$ & $3 * m * n$\\
     \hline
     \multirow{3}{*}{Commutative} & $A \odot B$ $^\ddag$ & $m * n$ & $B \odot A$ & $m * n$\\
     ~ & $ReduceSum(BitShift(A))$ $^\P$ & $2 * m * n$ & $BitShift(ReduceSum(A))$ & $m * n + m$\\
     ~ & $ReduceProd(Exp(A))$ $^\P$ & $2 * m * n$ & $Exp(ReduceSum(A))$ & $m * n + m$\\
     \bottomrule
     \multicolumn{5}{l}{{\scriptsize $^\S$ $B + 1$ are not counted in the \#FLOPS as 1 is constant value, so it does not need to load data from cache.}} \\
     \multicolumn{5}{l}{{\scriptsize $^\dag$ First using commutative property to swap the order of $B$ and $Abs(C)$, then applying associative property.}} \\
     \multicolumn{5}{l}{{\scriptsize $^\ddag$ Even though this pattern has no \#FLOPS gains, but it can enable further optimization in, e.g in $\dag$.}} \\
     \multicolumn{5}{l}{{\scriptsize $^\P$Suppose the reduce axis of ReduceSum/ReduceProd is inner-most dimension to calculate the \#FLOPS.}} \\
\end{tabular}
\end{table*}
\endgroup

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95 \textwidth]{figures/data_graph_opt.pdf}
    \caption{Data movement operators optimization. \bren{TODO: change sub-captions of each figure}}
    \label{fig:data-type-example}
\end{figure*}

\subsubsection{Fusion Plan Generation Algorithm}

List~\ref{lst:fusion-plan-generation} shows our detailed fusion plan exploration algorithm. \bren{Please notice this algorithm only generates the fusion plan (i.e., candidate fusion blocks) without performing the real fusion because the candidate fusion blocks will be further optimized by subsequent graph rewrite (as shown in Section~\ref{}) before the real fusion code generation.} Figure~\ref{fig:fusion-plan-generation} illustrates its basic idea with a simplified example. This algorithm consists of three main steps as follows:

\textcolor{red}{TODO: correct all line numbers, or label those lines and ref them in text}

\paragraph{Step I: Fusion seed operators selection.} \projectname selects the one-to-one operator with the minimum intermediate result as the  fusion seed operator  (as shown in Listing~\ref{lst:fusion-plan-generation} lines 24 to 28). \gagrawal{explain why choose the one with minimum intermediate result}. 
\bren{If multiple seed operators with a minimum size of intermediate results exist, \projectname initiates fusion with them one after another} \gagrawal{Seems to contradict choosing minimum intermediate result criteria - that should almost always reduce the choice to one} \bren{double-check this?} 
It is also possible that multiple seeds are grouped to the same candidate fusion block in one round, \projectname then initiates fusion plan generation with the rest ones.  In Figure ~\ref{fig:fusion-plan-generation}, {\tt Add}, {\tt Relu}, {\tt Mul}, and {\tt Sub} are in one-to-one type (with an identical intermediate result size), then {\tt Add} is selected as the seed for the first round of fusion plan exploration.

\gagrawal{let us decide and use only one name between consumers/successors and producers/predecessors}. 

\paragraph{Step II: Propagated fusion plan exploration along seed's consumers.} 
Each operator may have one or multiple producers and consumers. \projectname first processes the seed operator's consumers (Listing ~\ref{lst:fusion-plan-generation} Lines 1 to 18). This step consists of four sub-steps: First, {\em mapping type analysis} 
(Listing ~\ref{lst:fusion-plan-generation} Step 2.1) categorizes the potential fusion result into three types based on the operators mapping type and Table~\ref{tab:mapping-type-lookup}.  1) {\tt fuse\_break} indicates that fusion between these operators causes overhead, due to introduced memory or computation overhead (e.g. random memory accesses or redundant computations), 
thus fusion should be aborted (Red cases in Table~\ref{tab:mapping-type-lookup}); \gagrawal{are they still legal?} 2) {\tt fuse\_through} indicates that this fusion yields benefits and should be proceeded without any further analysis (Green cases in Table~\ref{tab:mapping-type-lookup}); 3) {\tt fuse\_depend} indicates that this fusion requires an extra experimental study with either our historical data in database, or a temporal fusion and deployment on runtime to check if fusion brings any benefit (Yellow cases in Table~\ref{tab:mapping-type-lookup}).  
Second, a further machine-independent constraints check (Listing ~\ref{lst:fusion-plan-generation} Step 2.2) is designed to analyze if this fusion incurs any overhead, e.g., increasing register usage, causing redundant computations, \wniu{too many random memory access}, or extra materialization, etc. Third, as aforementioned, an experimental study (Listing ~\ref{lst:fusion-plan-generation} Step 2.3) is required if the mapping relation is {\tt fuse\_through}. Fourth, \projectname continues processing the consumers of current consumers by repeating this step recursively until the analysis fails. Figure~\ref{fig:fusion-plan-generation} shows an example of fusing {\tt Add} with {\tt Conv} and the rest consumers with this step. After this step, the generated candidate fusion block is in a mapping type of many-to-one, and includes five operators ({\tt Add}, {\tt Conv}, {\tt Relu}, {\tt Mul}, and {\tt Sub}). 

\paragraph{Step III: Propagated fusion plan exploration along seed's producers.} After processing along the seed's consumers direction, \projectname processes along the seed's producers direction with the same algorithm as Step II. \gagrawal{explains why first consumers and then producers}.  In the example in Figure~\ref{fig:fusion-plan-generation}, the first attempt of fusing current candidate fusion block with {\tt GEMM}  fails because both of them are in many-to-one mapping type. Table~\ref{tab:mapping-type-lookup} indicates this is a {\tt fuse\_break} case, so {\tt GEMM} is not included in this candidate fusion block.  

\paragraph{Iterate.} \projectname completes a round of fusion plan generation with above steps. If more fusion seeds exist, it will iterate from Step II with the next seed until all seeds are consumed. 

\gagrawal{should we talk somewhere about how we deal with multiple consumers/producers of a node?}. 

% \wniu{
% As each starting point can be fused with its predecessor or successor, after traversing the consumer (successor), in step 3 (line 21), we head to producer (predecessor). The similar procedure happens in step 3. The only different thing is the fusion direction is reversed. 
% }

%\paragraph{Step IV: Continue from Step II for rest seeds.}\wniu{Does this need to be removed?}

% \lstset{numbers=left, numberstyle=\tiny, stepnumber=1, numbersep=5pt, frame=tb, caption=Graph rewriting,emph={},emphstyle=\underbar}
% \lstinputlisting[label={lst:graph-rewriting},language=python]{codes/graph-rewrite.py}

\subsection{Computation-property-based Graph Rewrite}
% Using evaluation to demonstrate this works better on extreme DNNs than shallow one. 
\gagrawal{why do fusion and then graph rewrite? It makes more sense to me to do rewrite and then fusion? and why are we limiting rewriting within a fusion block}
\bren{Good question. Let us discuss this. we can rewrite at first. this is also more interesting.}
After generating the fusion plan, \projectname employs a computation-property-based computational graph rewrite pass to further optimize the computation within each candidate fusion block. Figure~\ref{fig:fusion-type-example} (\wniu{the character below the operator means this operator has an extra input from model weights}) shows the leveraged computation properties (distributive, communicative, and associative).
With this graph rewrite, \projectname is able to 1) remove unnecessary operations (e.g., matrix/tensor reshape\wniu{Is this in Advanced opt?}), 2) eliminate redundant intermediate data copies, and 3) replace costly operators (or combinations of operators) with more efficient ones. 

The detailed definition and example of the graph rewrite based on each property is explained as follows:

\renewcommand{\labelenumii}{\Roman{enumii}}
\begin{itemize}[leftmargin=*,noitemsep,nolistsep]
\item {\bf Associative:}
By leveraging the associative property, the graph rewrite pass can identify an optimized order of operators execution, and hence replace the expensive combination of operators with a new cheaper one that yields an result identical to the original operators. Figure~\ref{fig:fusion-type-example} (a) shows an example, in which a combination of two {\tt Recip} operators and two {\tt Mul} operators is replaced by a combination of a {\tt Recip}, a {\tt Square}, and a {\tt Mul}. 
The latter is more efficient by simplifying and linearizing the computation.  In particular, it has two positive effects: first, it eliminates a {\tt Mul} operator; second, the intermediate result size is significantly reduced that will reduce the register pressure after subsequent fusion. 

\item {\bf Distributive:}
The basic idea of distributive property-based graph rewrite is similar to the one based on associative property. The only difference is to use the distributive property rather than associative property to guarantee the correctness of the transformation. As shown in Figure~\ref{fig:fusion-type-example} (b), the combination of two {\tt Mul} operators and an {\tt Add} can be replaced by an {\tt Add} followed by a {\tt Mul}. It mainly aims to eliminate the unnecessary operator.

\item {\bf Commutative:}
The property guaranties the legality of swapping the position of two operators, which usually results in computation reduction. As shown in Figure~\ref{fig:fusion-type-example} (c), {\tt BitShift} \footnote{Calculate the bit shifted value of elements of a given tensor element-wisely.} and {\tt ReduceSum}\footnote{Calculate the reduced sum of elements of an input tensor along an axis.} satisfy communicative property, thus {\tt ReduceSum} can be scheduled to execute before {\tt BitShift}. After this swap, 
unnecessary bit shifts can be reduced significantly. %For example, if the output shape of BitShift is ($m \times n$), and the axis of ReduceSum is 2, so the output shape of ReduceSum is $m \times 1$. That means bit shift need to be compute $m \times n$ times, after swap, only need to do $m \times 1$ times. The computation of ReduceSum keeps the same.
% 

%\textcolor{red}{TODO: Rewrite from here...}
\end{itemize}


%\textcolor{blue}{Mechanism: Each operator in our unified computational graph has a priority property (need to provide a table?), }

\projectname requires to figure out two major issues during this graph rewriting:

{\bf Issue I:} How to recognize the rewrite candidates in each candidate fusion block?

\projectname employs pattern matching~\cite{} \textcolor{red}{CITE} to recognize rewrite candidates. The major \wniu{or part?} available patterns are summarized in Table~\ref{tab:graph_rewrite_example}. This table also shows the computational graph structures (in equations), and the computation amounts (in \#FLOPS) before and after rewrite. This table mainly covers multiple operators in one-to-one mapping type (e.g., element-wise multiplication, addition, reciprocal, square root, etc.) and several reduction operators that are in many-to-one mapping type (e.g., {\tt ReduceSum} and {ReduceProd}) because these operators usually follow our defined computation property. This table is extensible and will cover more types of computations in the future.

{\bf Issue II:} In which order to perform the rewrite? 

\bren{TODO: change this to whole graph...}
Although associative and commutative matching is NP-complete~\cite{benanav1987complexity}, \projectname is still possible to explore all possible patterns and pattern combinations in each candidate block because most candidate blocks have limited number of operators. Table~\ref{tab:graph_rewrite_example} also lists the potential computation reduction with the graph rewrite following each pattern, which \projectname uses as its (simplified) cost model to determine the optimal rewrite plan.  
% \projectname employs the following heuristic approach. First, it scans all available patterns in each block, and identify the optimized sub-block after using graph rewrite (the optimization is implicate in the pattern). We compute the computation size before and after applying graph rewrite, then rank the matched pattern by their saved computation size. A pattern with the highest computation saving is selected, and marked as {\tt re-writed}. Then all the operator will be marked or no pattern can be found in the rest sub-block after we iteratively repeat the preceding steps.

%\textcolor{red}{TODO: mark a/b/c... in fig 2 to make the pointer more precisely.}


%\textcolor{red}{TODO: more algorithm aspects: 1) how to find the combinations satisfy these properties; 2) the order to apply them or the priority to apply them; 3) how can we say rewriting mainly works for One-to-one, Shuffle and Reorganize without side-effect.}




\subsection{Advanced Fusion-based Optimizations} 

\gagrawal{May be call it code generation and optimization and first talk about code generation?}. 

%\textcolor{red}{TODO: just some notes, will work on it next...}

Besides graph rewrite, \projectname also includes several advanced optimizations enabled by our fusion analysis and optimization. This section categorizes them into two types, intra-fusion-candidate-block  and inter-fusion-candidate-block optimizations.

\subsubsection{Intra-candidate-block Optimizations}
 
 Operators in shuffle and reorganize mapping types usually intensively manipulate data movement. 
 
 \bren{TODO: some notes, write this section from here.}
 
 the nest loop by split a operator to its raw definition and corresponding nested loop information. Also, computation based rewriting is not conflict with data based rewriting, as optimizing objects of computation based rewriting are data-computation operators, while the targets of data based rewriting are data movement operators.

\begin{enumerate}[leftmargin=*,noitemsep,nolistsep]
\item {\bf Data aggregation:}
This policy optimize the loop concatenate. In this step, we split the operator properties and definition from the data aggregation operators, then convert these information to loop transformation in our UCG. This can help us to generate code easily.

\item {\bf Data transportation:}
In data transportation policy, we can remove Transpose operator in the fused block, then embed the transpose information to its producer or consumer. In the embedding phase, more optimization can be explored especially when it consumer is computation intensive operator, e.g. MatMul, CONV.

\item {\bf Data splitting:}
The main purpose of data splitting is combining two different branch of sub-block. Similar with the data aggregation policy, this policy splits the nested loop information from the operator, then update our UCG to help generate more efficient code.

\end{enumerate}

\subsubsection{Inter-candidate-block Optimizations}
\paragraph{Layout transformation elimination.}
\textcolor{blue}{Data layout is critical to end-to-end performance. Remove transpose or layout transformation via fusion. Eliminate data layout transformation taken place in computation intensive operation and maintain the same data shape as far as possible. To keep computation more consistent way.}

\paragraph{Inter-operation optimization.} 
\textcolor{blue}{MatMul operation occupies most computation workload among BERT models, it also has Transpose and Reshape operation at the front of MatMul. So we can combine the intrinsic optimization of MatMul with Reshape and Transpose, e.g. Transposed matrix multiplication.}
\textcolor{blue}{CONV with Deconv: NCHW -> NHWC, data transpose.}


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.98 \columnwidth]{figures/code_gen_tree.pdf}
    \caption{Code generation.\bren{mark sub-figures with ECG, Data-flow tree, and Code generation}}
    \label{fig:code-generation-tree}
\end{figure}


\subsection{Bottom-up Fusion Code Generation}

 \projectname generates fused code for each candidate fusion block with a {\em data-flow tree} (DFT) built from the Extended Computational Graph (ECG). Figure~\ref{fig:code-generation-tree} shows an example. This DFT represents the final output ({\tt Out}), all intermediate results ({\tt IRS}), and all inputs ({\tt A}, {\tt B}, {\tt C}, and {\tt D}) with a bottom-up reversed traversal of ECG, meaning that the parent node depends on the children nodes. During the fused code generation, \projectname traverses this DFT in a breadth-first/depth-first manner to replace the parent node with its children nodes (and corresponding ECG operations), recursively. 
The right-hand side of Figure~\ref{fig:code-generation-tree}, shows an example of this replacement. First, $Out$ is replaced by $IRS_3 \ +\ IRS_5$; next, $IRS_3$ is replaced by reciprocal of $IRS_2$, and so on, until reaching the input of $A, B, C, D$. It is worth noting that \projectname can also find {\em redundant computations} in DFT with a common sub-tree identification and eliminate them during the code generation, e.g. both {\tt Mul} operators use $IRS_1$, resulting in a common sub-tree in DFT, thus the replacement in two red boxes of Figure~\ref{fig:code-generation-tree} is only generated once. \gagrawal{we should explain why we are making these choices}.  

%\textcolor{red}{TODO: rephrase, will work on it next...}

List~\ref{lst:code-generation} shows more details of \projectname's fusion code generation (that is actually a source-code-to-source-code transformation) that consists of four steps. Step 1 (Listing 2 Line 35) finds the final output (or outputs) in a candidate fusion block (e.g., {\tt Out} in Figure~\ref{fig:code-generation-tree}). 

\bren{TODO: Not clear this part and listing 2, revising...}
Note that, each output of a operator has and only has one producer which is the operator itself, while each operator can have more than one producer, as it may have multiple inputs. In step 2 (Listing 2 Line 38), we recursively replace the intermediate results by its producer until none of the intermediate results can be replaced (Listing 2 Line 27 to 28), the same thing happens when we replace $IRS_3$ by $Reciprocal(IRS_2)$. Then in step 3 (Listing 2 Line 25), we find the 
AST (Abstract Syntax Tree) for two operators, and merge them into the final AST by analyzing their mapping type. Finally, in step 4 (Listing 2 Line 4), if there are more than one output for a block, we merge the AST for each output. Until now, the code are generated.


\wniu{Key insight: bottom-up, IRS replacement. Explain why bottom-up, and how to deal with the index transformation for shuffle and reorganize, and how to handle different mapping type combine. }


% https://www.overleaf.com/learn/latex/code_listing
% \lstset{numbers=left, numberstyle=\tiny, stepnumber=1, numbersep=5pt, frame=tb, caption=Code generation}
% \lstinputlisting[language=python,label={lst:code-generation}]{codes/code-generation.py}


\subsection{\projectname Implementation}

%\textcolor{red}{TODO: we need to introduce this because we are doing an end-to-end performance comparison with other frameworks}

\projectname is implemented on an existing end-to-end DNN execution framework\footnote{The name and paper reference will be added later for anonymity  purpose.} that supports both dense and sparse DNN execution. \projectname is currently implemented on its version supporting dense DNN that performs similarly to TVM, MNN, and TFLITE without the operator fusion provided by \projectname. For readability, we also call this optimized framework \projectname. Next section introduces more comparison results between it and other frameworks.  

==> tex/draft.tex <==
\section{Drafts}

% Performance table, FLOPS != MACS
\begingroup
\setlength{\tabcolsep}{7.4pt}
\renewcommand\arraystretch{1.0}
\begin{table*}[t!]
\centering
\caption{{\bf Inference latency comparison: \projectname, MNN, TVM, TFlite, and PyTorch on mobile CPU and GPU.} \#FLOPS denotes the number of floating point operations. OurB is our baseline implementation by turning off all fusion optimizations and OurB+ is OurB with a fixed-pattern fusion as TVM. DNNF is short for \projectname, i.e., our optimized version. '-' denotes this framework does not support this execution.}
\label{tab:eva_performance_report}
\small
\begin{tabular}{l|cc|cc|cc|cc|cc|cr}
     \toprule
     \multirow{2}{*}{Model} & \multirow{2}{*}{\#Params} & \multirow{2}{*}{\#FLOPS} & \multicolumn{2}{c|}{MNN (ms)} & \multicolumn{2}{c|}{TVM (ms)} & \multicolumn{2}{c|}{TFLite (ms)} & \multicolumn{2}{c|}{Pytorch (ms)} & \multicolumn{2}{c}{{\bf DNNF (ms)}} \\ \cline{4-13}
     ~                  & ~ & ~  & CPU & GPU & CPU & GPU & CPU & GPU   & CPU   & GPU & {\bf CPU} & {\bf GPU} \\ \hline
     EfficientNet-B0    & 5.3M & 0.8B  & 41 & 26 & 56 & 27 & 52  & 30 & 76 & - & {\bf 16} & {\bf 10}  \\
     ResNet-50          & 26M &  8.2B & 124 & 47 & 143 & 64 & 135  & 57 & 188 & - & {\bf 82} & {\bf 38} \\
     VGG-16             & 138M & 31.0B & 242 & 109 & 260 & 127 & 245  & 102 & 273 & - & {\bf 171} & {\bf 65}  \\
     MobileNetV1-SSD    & 9.5M &  3.0B & 67 & 43 & 74 & 52 & 87  & 68 & 92 & - & {\bf 33} & {\bf 17} \\
     MobileNetV3        &   6M & 0.45B & 18 & 16 & 17 & 15 & 15  & 13 & 22 & - & {\bf 12} & {\bf 10} \\
     YOLO-V4            &  64M & 34.6B & 501 & 290 & 549 & 350 & 560  & 288 & 872 & - & {\bf 235} & {\bf 117} \\
     C3D                &  78M & 77.0B & 867 & - & 1,487 & - & - & - & 2,541 & - & {\bf 582} & {\bf 301} \\
     R2+1D              &  64M & 76.3B & - & - & - & - & - & - & 4,104 & - & {\bf 623} & {\bf 312} \\
     S3D                & 8.0M & 79.6B & - & - & - & - & - & - & 6,612 & - & {\bf 710} & {\bf 324} \\
     PointPillar        & 4.8M &   97B & 489 & 245 & - & - & -  & - & - & - & {\bf 357} & {\bf 183} \\
     U-Net              & 2.1M & 15.0B & 181 & 106  & 210 & 120 & 302 & 117 & 271 & - & {\bf 99}  & {\bf 52}  \\
     Faster R-CNN       &  41M & 47.0B & - & - & - & - & - & - & - & - & {\bf 862} & {\bf 531} \\
     Mask R-CNN         &  44M &  184B & - & - & - & - & - & - & - & - & {\bf 2,471} & {\bf 1,680} \\
     TinyBERT           &  15M &  4.1B & - & - & - & - & 97 & - & - & - & {\bf 51} & {\bf 30} \\
     DistilBERT         &  66M & 35.5B & - & - & - & - & 510 & - & - & - & {\bf 224} & {\bf 148} \\
     ALBERT             &  83M & 65.7B & - & - & - & - & 974 & - & - & - & {\bf 386} & {\bf 312} \\
     BERT$_\text{Base}$ & 108M & 67.3B & - & - & - & - & 985 & - & - & - & {\bf 394} & {\bf 293} \\
     MobileBERT         &  25M & 17.6B & - & - & - & - & 342 & - & - & - & {\bf 170} & {\bf 102} \\
     GPT-2              & 125M & 69.1B & - & - & - & - & 1,102 & - & - & - & {\bf 394} & {\bf 292} \\
     \bottomrule
\end{tabular}
\end{table*}
\endgroup
